Performance Quantification of a Nonlinear Model Predictive Controller by Parallel Monte Carlo Simulations of a Closed-loop System

This paper presents a parallel Monte Carlo simulation based performance quantification method for nonlinear model predictive control (NMPC) in closed-loop. The method provides distributions for the controller performance in stochastic systems enabling performance quantification. We perform high-performance Monte Carlo simulations in C enabled by a new thread-safe NMPC implementation in combination with an existing high-performance Monte Carlo simulation toolbox in C. We express the NMPC regulator as an optimal control problem (OCP), which we solve with the new thread-safe sequential quadratic programming software NLPSQP. Our results show almost linear scale-up for the NMPC closed-loop on a 32 core CPU. In particular, we get approximately 27 times speed-up on 32 cores. We demonstrate the performance quantification method on a simple continuous stirred tank reactor (CSTR), where we perform 30,000 closed-loop simulations with both an NMPC and a reference proportional-integral (PI) controller. Performance quantification of the stochastic closed-loop system shows that the NMPC outperforms the PI controller in both mean and variance.

==> tex/MC.tex <==
\section{Monte Carlo Simulation}





\begin{subequations}
	\begin{align}
		y_k &= g(t_k, x_k, p_g) + v_k, \\
		z_k &= h(t_k, x_k, p_h), \\
		x_k^c &= \kappa(t_{k-1}, x_{k-1}^c, y_k, u_{k-1}, p_{\kappa}), \\
		u_k &= \lambda(t_k, x_k^c, p_{\lambda} ), \\
		z_k^c &= \mu( t_k, x_k^c, p_{\mu}), \\
		x_{k+1} &= \Phi(t_k,x_k,u_k,d_k,w_k,p_f,p_\sigma),
	\end{align}
	\label{eq:closed_loop}
\end{subequations}
